MALT Powers Up Adversarial Attacks

Current adversarial attacks for multi-class classifiers choose the target class for a given input naively, based on the classifier's confidence levels for various target classes. We present a novel adversarial targeting method, \textit{MALT - Mesoscopic Almost Linearity Targeting}, based on medium-scale almost linearity assumptions. Our attack wins over the current state of the art AutoAttack on the standard benchmark datasets CIFAR-100 and ImageNet and for a variety of robust models. In particular, our attack is \emph{five times faster} than AutoAttack, while successfully matching all of AutoAttack's successes and attacking additional samples that were previously out of reach. We then prove formally and demonstrate empirically that our targeting method, although inspired by linear predictors, also applies to standard non-linear models.

==> 03-experimentaltargetting.tex <==
\section{Experiments}
\label{sec:experiments}
% \gilad{Take one model (best one?) and analyze the examples by: (1) Both we and Auto attack succeed, (2) We succeed, Autoattack fail, (3) We fail autoattack succeed, (4) Both fail. Analyze target in each of them.}

In this section, we compare the MALT attack (using a standard APGD attack) to the current state of the art AutoAttack. Our comparison is made to be compatible with RobustBench (\citet{croce2020robustbench}), which is the standard benchmark for testing adversarial robustness. Namely, we consider attack on CIFAR-100 (\citet{krizhevsky2009learning}) with an $\ell_\infty$ budget of $\epsilon= 8/255$ and on ImageNet (\citet{deng2009imagenet}) with an $\ell_\infty$ budget of $\epsilon= 4/255$. We compare the two attacks on several robust models from the top RobustBench benchmark. 

For MALT, we consider calculating the score for the $c=100$ classes with the highest model's confidence and attacking the top $a=9$ classes according to this score. This corresponds to the targeted attacks in AutoAttack, which attempt to attack the top $9$ classes according to the model's confidence. All the hyperparameters of APGD and the other attacks used in AutoAttack are set to their default values. Full details for all experiments in this section are in \appref{appendix:experimentdetails}.

In \tabref{table:cifarpetsuccess} (CIFAR-100) and \tabref{table:imagenetpetsuccess} (ImageNet), we present the results of the experiments. Note that MALT is able to attack more images than AutoAttack across all robust models and for both datasets. Also, there is an inclusion of successful attacks in the sense that for every image that AutoAttack successfully attacks, MALT also succeeds. Thus, the improvement contains only images that AutoAttack fails on.
Note that in \tabref{table:imagenetpetsuccess}, the robust and clean accuracy is not exactly equal to those reported on the RobustBench website since newer versions of the Python libraries in use give slightly different results.
% (all results reported were measured in the same environment). Extra experiment details and results are in \appref{appendix:experimentdetails}.



% The section presents the results using the new targeting method with the well-known and fast APGD targeted attack (\cite{croce2020reliable}). We compare our specially targeted attack to the state of the art AutoAttack, consisting of four parameter-free attacks: targeted and untargeted APGD, targeted FAB attack (\cite{}), and untargeted Square attack (\cite{}). In our comparison, one can see the importance of targeting - the PET targeting algorithm improves the number of successful attacks. Images that were previously attacked using other targets and failed are now successfully attacked while replacing only the chosen targeting method. In addition, we mention the much shorter attack time - while AutoAttack performs multiple slower attacks, we show that a single and fast attack suffices with improved targeting.


% \begin{figure}[tbh!]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.7\columnwidth]{figs/petargeting/Liu2023Comprehensive_Swin-L/677.png}}
% \caption{PET targeted attack on Swin-L robust model from \cite{liu2023comprehensive}. We use $L_\infty$ attack with a budget of 4/255.}
% \label{fig:toaster}
% \end{center}
% \vskip -0.2in
% \end{figure}

% In \tabref{table:cifarpetsuccess} and \tabref{table:imagenetpetsuccess}, we present the total robust accuracy achieved by the two attacks. As mentioned in the complexity analysis in \secref{sec: method}, we consider only $c = 100$ optional classes: (1) for CIFAR100, we take all $100$ classes, and (2) for IMAGENET, for any image $x$, we take the $100$ classes corresponding to the top $100$ logits of $N(x)$. In addition, we take the top $a = 9$ best targets out of the $100$ considered, similar to the nine targeted attacks performed in AutoAttack. Note that in \tabref{table:imagenetpetsuccess}, the robust and clean accuracy is not equal to the reported on the RobustBench website since newer versions of the Python libraries in use give slightly different results (all results reported were measured in the same environment). Extra experiment details and results are in \appref{appendix:experimentdetails}.


\begin{table}[h!]
 \caption{\textbf{CIFAR100 - $L_\infty$} robust accuracy \emph{(lower is better)}, comparing MALT and AutoAttack, which is the current state of the art. 
 % rate using MALT targeting for the best 9 targets. Compared to the best-reported accuracy of the model via RobustBench (\cite{croce2020robustbench})
 }
 \label{table:cifarpetsuccess}
\begin{center}
\begin{small}
\begin{sc}
    
\begin{tabular}{|l |l |l |l | l| l |} 
 \hline
  \multicolumn{1}{|c|}{\bfseries Model} & \multicolumn{1}{|c|}{\bfseries} & \multicolumn{4}{|c|}{\bfseries  Robustness} \\
 \hline
   &  acc. & MALT & SOTA & diff & speed-up \\ 
  \hline
  %38.83 , 38.82, 38.79, 38.81, 38.82, 
WRN-28-10   \citep{wang2023better} & $72.58\%$ & $38.79\%$ & $38.83\%$ & \textcolor{green}{$-0.04\%$} & $\times $ $3.36$ $\pm0.18$ \\
 \hline
 % 42.66 , 42.68, 42.67, 42.69, 42.66
WRN-70-16 \citep{wang2023better} & $75.22\%$ & $42.66\%$ & $42.67\%$ & \textcolor{green}{$-0.01$\%} & $\times $ 3.87 $\pm0.08$\\
\hline
% 39.19, 39.20, 39.19, 39.19, 39.21
WRN-28-10 \citep{cui2023decoupled} & $73.83\%$ & $39.18\%$ & $39.18\%$ & \textcolor{black}{$0$\%} & $\times $ $3.43$ $\pm0.08$\\
 \hline
 % 36.81, 36.84, 36.84, 36.83, 36.82
WRN-70-16  \citep{gowal2020uncovering} & $69.15\%$ & $36.81\%$ & $36.88\%$ & \textcolor{green}{$-0.07$\%} & $\times $ $3.42$ $\pm0.09$\\

 \hline

    \end{tabular}


 \end{sc}
\end{small}
\end{center}
\end{table}


\begin{table}[h!]
 \caption{
 \textbf{ImageNet - $L_\infty$} robust accuracy \emph{(lower is better)}, comparing MALT and AutoAttack, which is the current state of the art.
 % For IMAGENET -$L_{\infty}$ APGD robust accuracy \textbf{(lower is better)} rate using MALT targeting for the best 9 targets. Compared to Standard AutoAttack robust accuracy
 }
 \label{table:imagenetpetsuccess}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{|l |l |l |l | l | l|} 
 \hline
   \multicolumn{1}{|c|}{\bfseries Model} & \multicolumn{1}{|c|}{\bfseries} & \multicolumn{4}{|c|}{\bfseries  Robustness} \\
 \hline
   &  acc. & MALT & SOTA & diff. & speed-up \\ 
  \hline
  Swin-L \citep{liu2023comprehensive}&  $79.18\%$ &  $59.84\%$ &  $59.90\%$ & \textcolor{green}{$-0.06\%$} & $\times$ $5.18$ $\pm0.04$\\
 \hline
  ConvNeXt-L \citep{liu2023comprehensive}&  $78.20\%$ &  $58.82\%$ &  $58.88\%$ & \textcolor{green}{$-0.06\%$} & $\times$ $5.22$ $\pm0.1$\\
  \hline
  ConvNeXt-L+ 
  % + ConvStem 
  \citep{singh2024revisiting}& $77.02\%$ &  $57.94\%$ & $57.96\%$ & \textcolor{green}{$-0.02\%$} & $\times$ $4.86$ $\pm0.06$\\
  \hline
    Swin-B \citep{liu2023comprehensive}& $76.22\%$ &  $56.54\%$ & $56.56\%$ & \textcolor{green}{$-0.02\%$} & $\times$ $5.02$ $\pm0.03$ \\
  \hline
 ConvNeXt-B+ 
 % + ConvStem 
 \citep{singh2024revisiting}& $76.00\%$ & $56.48\%$ & $56.52\%$ & \textcolor{green}{$-0.04\%$} & $\times$ $5.00$ $\pm0.07$\\

 \hline


    \end{tabular}
 \end{sc}
\end{small}
\end{center}
\end{table}

% \gilad{TODOs: (1) More examples of "toaster", i.e. targeting below top 10. (2) Our attack on all 1000 classes. (3) Our attack on top 10 (9?) divided by which class succeeded - bar figure. (4) Timing auto attack compared to ours on the first in each table of CIFAR100 and imagenet. (5) Figure out what happens with the third experiment on imagenet.}

\paragraph{Attack Running Time}
For the speed-up column, we first sampled uniformly from the test dataset five batches of size $200$ for ImageNet and $400$ for CIFAR100, which corresponds to $5 \times 4\%$ of the entire test set.
We timed both MALT and AutoAttack, when running on the exact same GPU chip and on the same samples, we present the mean and variance of these experiments for each robust model.
% took five random samples of each dataset. 
% We tested both attacks on each model for each sample, taking an average and variance over the samples.
On the ImageNet dataset there is on average a five times speed up, while for CIFAR100 it is $3.5$ times on average.
The lower rate can be explained by the higher attack success rates for CIFAR100. In other words, the complexity analysis from \secref{sec: method} is of the worst case, and since fewer test examples pass through all four different attacks in AutoAttack, the running time is lower.

% In \tabref{table:imagenetpetsuccess} we show up to five times speed up for, and slightly lower speed up rate for CIFAR100 in \tabref{table:cifarpetsuccess}. The lower rates for CIFAR100 explained by our worst-case running time analysis from \secref{sec: method}. As in CIFAR100 the attack success rates are higher (corresponds to a lower robust accuracy), fewer test examples passed throw all four AutoAttack attacks, speeding up the total running time.
% We also compared the running time of MALT with AutoAttack on the entire Imagenet test set, containing $5000$ images. MALT took $15$ hours and $8$ minutes to run, while AutoAttack took $62$ hours and $45$ minutes. Hence, MALT improves the running time by more than \emph{four times} over AutoAttack, in addition to improving the successful attacks.
%cifar attack is better since it succeeds more



\paragraph{Integrating MALT with different attacks}
Our experiments found that MALT operates well across datasets and models with the standard and fast APGD attack. We also integrated MALT with the targeted FAB attack (\citet{croce2020minimally}) on the Swin-L robust model (\citet{liu2023comprehensive}). This attack achieved a worse result of $60.64\% $ robust accuracy than using APGD with the DLR loss. 
% For this experiment, we followed our targeting algorithm with FAB attack, getting slightly worse results of 60.64\% robust accuracy for \citep{liu2023comprehensive} Swin-L network, higher (therefore less successful attack) than when using $APGD_{DLR}$.

% Running on one GPU of A100, our attack on the $5000$ images taken from the test set of IMAGENET lasted 15 hours and 8 minutes, while AutoAttack lasted two days, 14 hours, and 45 minutes.

\begin{wrapfigure}[24]{tbh!}{0.4\textwidth}
% \begin{figure}[tbh!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.4\columnwidth]{figs/petargeting/Liu2023Comprehensive_Swin-L/attack-saturated3.PNG}}
\caption{Comparing targeting methods for \citet{liu2023comprehensive} SOTA model: The number of successful attacks for each target order by two targeting methods: In blue, we use MALT targeting and APGD, and in orange, we compare to APGD with top logits targeting performed in AutoAttack.}
\label{fig:bars}
\end{center}
\vskip -0.2in
% \end{figure}
\end{wrapfigure}


\subsection{Targeting analysis}
In this subsection, we analyze the targeting mechanism of MALT and whether other targeting techniques could have improved it.
In \figref{fig:bars}, we show how the successful attacks are distributed according to the score given either by MALT or the naive targeting (i.e., according to the model's confidence). It is evident that the score provided by MALT leans much more towards the top -- $1$ than naive targeting. This indicates that the score provided by MALT has a higher correlation with successful attacks than the naive targeting method. Also, since MALT successfully attacks more images for the top $9$ targets, the sum over the columns of MALT attacks is larger than that of the naive targeting.



% Also note, that since in this figure we only considered the top $9$ classes using each score, the sum over the columns of the MALT attacks results in a larger number than that of the naive targeting.



Finally, we test whether the choice of $c=100$ is enough, namely calculating the score for MALT only for the top $100$ classes sorted by the confidence level of the model. To this end, we ran MALT with $c=1000$ for the ImageNet test dataset on the Swin-L robust network. Note that the number of gradient calculations for each test image has increased by a factor of more than two. This attack reached a robust accuracy of $59.84\%$, \emph{exactly the same as $c=100$}. This means that calculating the score for the top $100$ classes is enough to find the top classes to attack. It may be possible to optimize this hyperparameter even more, although the benefit in running time will be negligible. 

% taking the top-$9$ classes according to the score given by MALT exhaust all the possible target classes for the entire dataset, at least for the APGD attack.


% there may exist a better targeting method than MALT. 


% To this end, we ran a targeted APGD attack on the Swin-L robust network, for the entire ImageNet test dataset and for all the possible classes. Note that the test dataset consists of $5000$ images, each with a possible $1000$ classes. This attack reached a robust accuracy of $59.84\%$, \emph{exactly the same as MALT}. This means that taking the top-$9$ classes according to the score given by MALT exhaust all the possible target classes for the entire dataset, at least for the APGD attack.



% In orange, we show the successful AutoAttack attacks for each ordered target, from the first target chosen to the ninth. In blue, we show the same for the PET targeting method, demonstrating most of the first-picked targets led to a successful attack, and only a few more were added in the extra eight tries.


% We show that even though we try to .attack $a=9$ targets, most successful attacks are successful towards the first chosen targets. In \figref{fig:bars}, we show how the successful attack is distributed in terms of different target tries. In orange, we show the successful AutoAttack attacks for each ordered target, from the first target chosen to the ninth. In blue, we show the same for the PET targeting method, demonstrating most of the first-picked targets led to a successful attack, and only a few more were added in the extra eight tries.



% \subsection{Attack variances}
% \paragraph{Calculate scores for a larger portion of potential targets}
% We tested our targeting algorithm with $APGD_{DLR}$ with the SOTA robust network of \citep{liu2023comprehensive} Swin-L when choosing $c = k = 1000$. Meaning, we calculated the score for all the potential target classes. This attack is, of course, much slower, adding 900 backward passes to the previous calculations (for a total of 2801 passes). However, it doesn't achieve any better results, reaching 59.84\% robustness, as for the case $c=100$.

% \paragraph{Integrate PET with different attack}
% For this experiment, we followed our targeting algorithm with FAB attack, getting slightly worse results of 60.64\% robust accuracy for \citep{liu2023comprehensive} Swin-L network, higher (therefore less successful attack) than when using $APGD_{DLR}$.






% APGD - one backword and one forward for each step (100) - total of 1000 back and 1000 forwards (9 targets + untargeted)
% FAB - another 900 back and another 1827 forward (927 more than backwords, 103 per target)
% our algorithm by the total number of calls of the classifier
% Niter × Nrestarts ×(2×forward passes+ 1×backward pass)
% Per restart one has to add the three forward passes for the
% final search.
% square - 5000 steps forwards (implemented with 5001)
